Exploiting Inter- and Intra-Memory Asymmetries for Data Mapping in Hybrid Tiered-Memories

Modern computing systems are embracing hybrid memory comprising of DRAM and non-volatile memory (NVM) to combine the best properties of both memory technologies, achieving low latency, high reliability, and high density. A prominent characteristic of DRAM-NVM hybrid memory is that it has NVM access latency much higher than DRAM access latency. We call this inter-memory asymmetry. We observe that parasitic components on a long bitline are a major source of high latency in both DRAM and NVM, and a significant factor contributing to high-voltage operations in NVM, which impact their reliability. We propose an architectural change, where each long bitline in DRAM and NVM is split into two segments by an isolation transistor. One segment can be accessed with lower latency and operating voltage than the other. By introducing tiers, we enable non-uniform accesses within each memory type (which we call intra-memory asymmetry), leading to performance and reliability trade-offs in DRAM-NVM hybrid memory. We extend existing NVM-DRAM OS in three ways. First, we exploit both inter- and intra-memory asymmetries to allocate and migrate memory pages between the tiers in DRAM and NVM. Second, we improve the OS's page allocation decisions by predicting the access intensity of a newly-referenced memory page in a program and placing it to a matching tier during its initial allocation. This minimizes page migrations during program execution, lowering the performance overhead. Third, we propose a solution to migrate pages between the tiers of the same memory without transferring data over the memory channel, minimizing channel occupancy and improving performance. Our overall approach, which we call MNEME, to enable and exploit asymmetries in DRAM-NVM hybrid tiered memory improves both performance and reliability for both single-core and multi-programmed workloads.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> sections/new.tex <==
% \begin{figure*}[t!]%
%     \centering
%     \subfloat[]{{\includegraphics[width=6cm]{images/motivation/xz.pdf} }}%
%     %\qquad
%     \subfloat[]{{\includegraphics[width=6cm]{images/motivation/xz.pdf} }}%
%     %\qquad
%     \subfloat[]{{\includegraphics[width=9cm]{images/motivation/xz.pdf} }}%
%     \caption{Illustrating the trade-off between charge pump aging and SNN performance, considering PCM crossbars.}%
%     \label{fig:cp_motivate}%
% \end{figure*}



% \begin{figure*}
% \centering
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \captionof{figure}{A figure}
%   \label{fig:test1}
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \captionof{figure}{Another figure}
%   \label{fig:test2}
% \end{minipage}
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \captionof{figure}{A figure}
%   \label{fig:test1}
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \captionof{figure}{Another figure}
%   \label{fig:test2}
% \end{minipage}
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \captionof{figure}{A figure}
%   \label{fig:test1}
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \captionof{figure}{Another figure}
%   \label{fig:test2}
% \end{minipage}
% \end{figure*}




Figure \ref{fig:tms} illustrates a tiered memory system with heterogeneous memory nodes comprising of DRAM and PCM to combine the best properties (latency, endurance, energy) of these two memory technologies \cite{panabaker2010hybrid}. Non-volatile 3D Xpoint\footnote{3D Xpoint hybrid memory is widely believed to be a combination of DRAM and PCM, and is marketed under brand names Optane (Intel) and QuantX (Micron).} memory \cite{hady2017platform,bourzac2017has} is one such example of main memory systems where DRAM and NVM (e.g., PCM) are placed on separate DIMMs, sharing a common memory address space \cite{standard2005double,jedecnvdimm2017}. IBM Power9 processor \cite{sadasivam2017ibm} is another example where DRAM is used as write cache for PCM main memory \cite{chinnaswamy2014hybrid}. Regardless of the configuration, these systems support efficient tiering of data between heterogeneous memory nodes. For instance, to address PCM's limited write endurance, write intensive memory pages (called \emph{hot pages}) can be profiled and migrated to DRAM, during a program execution \cite{yan2019nimble,kumar2019dynamic}.
%to address PCM's limited write endurance
%Regardless of the configuration of heterogeneous memory systems, performance optimization involves placing memory pages to favourable memory nodes. For instance, to address endurance, write-intensive pages can be migrated to DRAM (which has unlimited write endurance), keeping all other pages to PCM.

\begin{figure}[t!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/Tiered_Memory_System.pdf}}
	\vspace{-10pt}
	\caption{Architecture of heterogeneous tiered memory systems.}
	\vspace{-10pt}
	\label{fig:tms}
\end{figure}

In addition to tiering between heterogeneous memory nodes, we introduce the memory architecture to support tiering within each memory node. In a recent work, Lee et al. \cite{lee2013tiered} propose the tiering concept for DRAM subarrays. We extend this concept to PCM partitions and evaluate its impact on performance, reliability, and energy. The memory architecture is shown to the right of Figure~\ref{fig:tms}. In this architecture, isolation transistors are inserted into a bitline to divide it into two segments -- near segment, which contains memory cells that are connected directly to the peripheral circuit, and  far segment, which contains memory cells that are connected to the peripheral circuit through the isolation transistor. We evaluate the effect of varying the size of near segments in Section \ref{sec:results}.

To access a memory cell in the near segment, the isolation transistor is turned off, causing the peripheral circuit to drive current through a reduced electrical load. This has two implications: 1) the cell can now be accessed faster (improving performance for both DRAM and PCM), and 2) current through the cell is lowered (improving reliability and reducing disturbance errors for PCM).
To access a memory cell in the far segment, the isolation transistor is turned on. The access latency of cells in the far segment is similar to the baseline architecture (without isolation transistors). In Section \ref{sec:allocation} we describe how \tech{} uses tiering to place memory pages in correct segments during their initial allocation.

\subsubsection{Latency Analysis}

\subsubsection{Reliability Analysis}
\label{sec:nvm_reliability}

\subsubsection{Energy Analysis}

\subsection{Storing First-touch Instructions: Bloom Filters}
\label{sec:storing}
The memory controller must store the set of most access inducing first-touch instructions from the execution phases in the FTI cache. A naive approach of implementing the FTI cache would be using a table of rows for first-touch instructions. However, the exact number of rows in the table will vary depending on the number of first-touch instructions and the number of memory accesses they induce, both of which are specific to the application being executed. If a table's capacity is inadequate to store all high access inducing first-touch instructions, \tech{} will start predicting every new first-touch instruction as non access-intensive, once the table is full. The OS page fault handler will allocate all new pages to the far memory segment, providing no significant performance improvement. Figure \ref{fig:access} reports the intensity prediction accuracy of 21 workloads (see Section \ref{sec:evaluation}) with FTI table of 32 and 128 entries. We make the following observation. Workloads such as bwaves and exchange2 have fewer than 32 access-intensive first-touch instructions. Therefore, we see no increase in the prediction accuracy when increasing the number of entries in the FTI table from 32 to 128. On the other hand, we see a significant improvement in accuracy for cam4, gcc, roms, and wrf with larger table size due to the presence of large number of access-intensive first-touch instructions in these workloads. We conclude that tables must be sized conservatively (i.e. assuming the maximum number of first-touch instructions in the evaluated workloads), leading to a large hardware cost for table storage. We propose to use bloom filer to implement FTI table, which we describe next.

\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/access.pdf}}
	\vspace{-10pt}
	\caption{Intensity prediction as a function of FTI table size.}
	\vspace{-10pt}
	\label{fig:access}
\end{figure}

A Bloom filter \cite{bloom1970space} is a data 
structure that provides a compact and memory-efficient way representing of set membership. 
% We will expand on this in Section \ref{sec:results}.

% Therefore, tables must be sized conservatively (i.e. assuming a large number of first-touch instructions), leading to large hardware cost for table storage. 

% To size the FTI cache conservatively and st


\subsection{Page Allocation in Tiered Memory System}
\label{sec:allocation}


% \begin{figure*}[t!]
% \centering
% \begin{subfigure}{.49\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \caption{A subfigure}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{.49\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \caption{A subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% \begin{subfigure}{.49\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \caption{A subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% \begin{subfigure}{.49\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \caption{A subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% \begin{subfigure}{.49\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \caption{A subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% \begin{subfigure}{.49\textwidth}
%   \centering
%   \includegraphics[width=.99\linewidth]{images/motivation/xz.pdf}
%   \caption{A subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{A figure with two subfigures}
% \label{fig:test}
% \end{figure*}

==> sections/observation.tex <==
%To mitigate the long latency,
We discuss our observations that
%We make 
%the following observations that 
lead to \tech{}.
\subsection{Idea: Segmented Bitline Architecture}

\noindent\textit{\underline{Observation 1}: A considerable portion of the latency and reliability bottleneck is not necessarily intrinsic to any specific memory technology, but often due to a deliberate trade-off made by memory designers to optimize cost per bit.}

This is observed and reported for DRAM \cite{lee2013tiered}. We expand this observation for NVM,  where each bit is represented by the resistance of a cell (low resistance \ineq{\rightarrow} `1' and high resistance \ineq{\rightarrow} `0'). 
The resistance is read and programmed by driving a rated current through the cell using a peripheral circuit, which consists of sense amplifiers (to read) and write drivers (to write). We analyze the internal architecture of a NVM bank and find that its peripheral circuit is several orders of magnitude larger than the size of a NVM cell~\cite{cho2005programming,dray2018high,sandhu2018memory,song2019enabling}.\footnote{NVM, like DRAM, is organized hierarchically. An example NVM of 128GB capacity has 4 {channels}, with 4 ranks per channel, and 8 banks per rank. A bank has {8} {partitions}, which are similar to subarrays in DRAM.} To amortize this large size, memory designers connect a peripheral circuit to many (typically 4096) NVM cells through a wire called a \textit{bitline}. Numerous bitlines are laid in parallel to form a NVM array. A row of NVM cells is called a \emph{wordline}. 

Figure~\ref{fig:cost_per_bit} plots the design analysis performed while architecting main memory systems. The left subfigure shows such analysis for PCM, an emerging NVM, based on Micron's 45nm design~\cite{pcm_book}.\footnote{We expect the values to be of similar orders of magnitude for other designs.} The left y-axis plots the IR drop (explained below) on the bitline for SET, RESET, and READ operations as a function of the number of bitline cells. The right y-axis plots the normalized cost per bit. We observe that the normalized cost decreases as the number of bitline cells increases. However, higher the number of bitline cells, higher is the IR drop, meaning that higher is the latency and reliability degradation. The trade-off point is typically set to 4096 cells in most designs~\cite{pcm_book,lung2016double,redaelli2017semiconductor,villa2018pcm}.

\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/cost_per_bit.pdf}}
	\caption{Design analysis pertaining to the length of bitlines in NVM (e.g., PCM) and DRAM banks.}
	\vspace{-10pt}
	\label{fig:cost_per_bit}
\end{figure}

%\vspace{-10pt}


The right subfigure of Figure~\ref{fig:cost_per_bit} plots the analysis for DRAM, based on Micron's 45nm design~\cite{lee2013tiered,das2018vrl}. The figure plots the increase in row-conflict latency \ineq{tRC} (left y-axis) and the decrease in design cost (right y-axis) as a function of the number of bitline cells in a DRAM subarray. For DRAM, the trade-off point is 512 cells. We assume, without loss of generality, each bitline in NVM and DRAM contains 4096 and 512 cells, respectively.

Figure~\ref{fig:bitline} shows a bitline represented as a lumped RC parasitic circuit with NVM cells connected at the bitline's intersection with wordlines. %For discussion purposes, we only show the nearest and the farthest NVM cells. 
To access (i.e., to set, reset, or read) a cell, the voltage on the wordline is raised, connecting the cell's resistance to the bitline. Subsequently, the peripheral circuit (shown at the bottom of the bitline) drives current through the cell using a bias voltage (\ineq{V_\text{bias}}), which is higher than the IR drop on the bitline.

\begin{minipage}[h]{0.46\columnwidth}
\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/cell_structure.pdf}}
	%\vspace{-10pt}
	\captionof{figure}{Bitline parasitics.}
	\label{fig:bitline}
\end{minipage}
\begin{minipage}{0.46\columnwidth}
	\renewcommand{\arraystretch}{1.0}
	\setlength{\tabcolsep}{1.0pt}
	\centering
	{\fontsize{8}{10}\selectfont
    \begin{tabular}{c|cc}
    \hline
    \textbf{Cell} & \multicolumn{2}{|c}{\textbf{Bias Voltage}} \\ \cline{2-3}
    \multirow{2}{*}{\textbf{Op.}} & \textbf{Long bitline} & \textbf{Short bitline}\\
    & \textbf{(4096 cells)} & \textbf{(512 cells)}\\
    \hline
    \textit{Set} & 3.7V & 2.3V  \\
    \textit{Reset} & 7.1V & 6.9V\\
    \textit{Read} & 2.85V & 1.2V \\
    \hline
    \end{tabular}}
    \captionof{table}{Biasing Voltages.}
	\label{tab:bias}
\end{minipage}

\vspace{6pt}
%. To drive the rated current through the cell, the bias voltage must compensate the entire IR drop on the bitline.

%a current source (shown at the bottom) drives a current through the bitline to generate the required \textit{bias voltage} across the cell, while  compensating for IR drop on parasitic components in its path. %The farther a cell is from the current source, the higher is the IR drop and therefore, slower it is to access. 
%on the nearest and farthest cell 

Table \ref{tab:bias} reports minimum bias voltages required for set, reset, and read operations, respectively, in Micron's 45nm PCM device with transistor-switched cells~\cite{pcm_book}. Voltage values are reported considering long (4096 cells) and short (512 cells) bitlines. For diode-switched cells, the bias voltages are even higher due to the diode's high built-in potential. 

In contrast, each DRAM bit is represented by charge on a capacitor.
DRAM accesses are facilitated by charge sharing (rather than current conduction as in NVM). Therefore, the highest operating voltage of a DRAM cell is much lower. 

Setting aside the \textit{latency impact} due to parasitic capacitance on long bitlines in a NVM device, which is also observed and reported for commodity DRAMs~\cite{lee2013tiered,chang2016understanding}, there is also the high-voltage-related reliability impact in NVM, especially for the CMOS structures in its peripheral circuit~\cite{balajical19}.



%These results have two implications. First, long bitlines lead to higher latency. Second, high voltage operations lead to reliability issues of CMOS structures in a peripheral circuit \cite{balajical19}.


% Unfortunately, to access any cell on the bitline, the peripheral circuit needs to compensate for IR drop on the entire bitline. This means that 
% %To reduce design complexity, a conservative approach 
% %by default always programming 
% the highest voltage must always be programmed on the bitline, i.e., 5.7V to Set, 13.1V to Reset, and 3.85V to Read, irrespective of the distance of the accessed cell from the peripheral circuit.

% This means that nearby cells can be accessed
% The farther a cell is from the current source, the higher is the IR drop and therefore, slower it is to access. 
% This means that cells that are closer to the current source are overdriven, leading to their higher aging. In Section \ref{sec:nvm_reliability} we formulate the aging of a NVM cell, as a measure of its reliability.



\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/splitted_bitline.pdf}}
	\caption{(a) Bitlines partitioned into segments. (b) Accessing a near segment cell. (c) Accessing a far segment cell.}
	\vspace{-10pt}
	\label{fig:splitted_bitline}
\end{figure}
%Figure \ref{fig:splitted_bitline}(c) shows  In this way, cells in the near segment can be accessed faster with lower bias voltages, i.e., with higher reliability. 
%\vspace{-6pt}

%to achieve low cost-per-bit, while allowing
Observation 1 leads to our \textbf{first key idea} of introducing isolation transistors on long bitlines in a NVM device to allow their lengths to appear shorter, thereby achieving low latency and high reliability, without increasing the cost per bit. 
Figure~\ref{fig:splitted_bitline}(a) shows the proposed architecture (details in Section~\ref{sec:architecture}), where each long bitline is split into two segments using an isolation transistor: the segment connected directly to the peripheral circuit is called the \textit{near segment}, whereas the other is called the \textit{far segment}. 
Cells in the near segment can be accessed faster using lower bias voltages due to reduced parasitics on the current path (Figure~\ref{fig:splitted_bitline}(b)).
%(of the near segment instead of the entire bitline)

However, the isolation transistor increases access latency of the far segment and introduces 
%a resistance --- 
its ON resistance 
%of the isolation transistor 
%--- 
in the current path, which imposes additional bias requirement for the peripheral circuit (Figure~\ref{fig:splitted_bitline}(c)). This lowers reliability of the peripheral circuit in accessing the far segment. %Bitline segmentation was first proposed for DRAM~\cite{lee2013tiered}. We extend the concept to NVM and address the associated performance and reliability trade-offs.%, where authors show a significant performance improvement

\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/perf_observation_1.pdf}}
	\caption{Execution time of our evaluated workloads normalized to Baseline where bitlines are not segmented.}
	\vspace{-10pt}
	\label{fig:observation_1}
\end{figure}

%\vspace{-10pt}

Figure~\ref{fig:observation_1} plots the execution time of 15 workloads (see Section~\ref{sec:evaluation}) on a hybrid memory architecture with segmented bitlines. Results are normalized to the execution time of a Baseline design, where bitlines are not segmented. We observe that simply introducing segments in each bitline is just not enough to guarantee performance improvement; in fact, performance improves by only 2\% on average for these workloads.
We believe that our hybrid tiered-memory architecture can deliver on its promises if the inter- and intra-memory asymmetries are exploited efficiently by 
%cannot deliver on its promises significantly unless supported 
an operating system (OS) level page management policy.

\subsection{Idea: Intelligent Page Placement}
% with segmented bitlines introduces \textit{inter- and intra-memory performance and reliability asymmetries},
% which need to be exploited efficiently by 
% %cannot deliver on its promises significantly unless supported 
% an operating system (OS) level page management policy to deliver on the promises. 

We now shift our discussion to OS implementations.
Modern OSes 
% are already aware of inter-memory performance and reliability asymmetries in allocating and migrating memory pages.
% We now look at OS page allocation and migration policy for hybrid memoies.
% To explain our proposed page allocation policy, we first introduce the current state-of-the-art in OS support for hybrid memories.
% A modern OS such as Linux 
implement first-touch page allocation policy, where a virtual-to-physical address translator allocates a random physical memory page from the free pool to a virtual page address, when the virtual page is first touched by a memory instruction in the program. We call this instruction \textit{first-touch instruction} (\textbf{FTI}).
Many modern OSes are already aware of inter-memory performance and reliability asymmetries.
For instance, 
%Existing page management policy such as 
Nimble~\cite{yan2019nimble} starts with the default OS page allocator to assign a random physical page to a virtual address during its initial allocation~\cite{kumar2019dynamic}. Subsequently, Nimble re-allocates pages during program execution, based on continuous feedback received from the memory-side cache monitoring unit. In this way, Nimble can migrate an access-intensive page, called \textit{hot page}, to a fast memory, e.g., DRAM, if the page is not already placed there during its initial allocation~\cite{blagodurov2019hot}. There are three key drawbacks associated with this approach. First, Nimble incurs significant performance and energy overhead due to the high bank and channel occupancy during movement of data between memories. Second, access intensity of memory pages vary over time during the program execution. To effectively utilize the fast memory, Nimble de-allocates a previously migrated hot page that has been cold for a while to a slow memory to make space for new hot pages that may appear in the program. This is particularly observed for applications with irregular memory accesses. Third, a page's re-allocation and de-allocation from a memory incurs performance overhead in updating page table entries \cite{pham2015large,BhattacharjeeASPLOS}.

We make the following observations regarding page allocation and dynamic page migration in hybrid memories.

\noindent\textit{\underline{Observation 2}: A significant number of pages in a program are migrated more than once during execution.}

Figure~\ref{fig:migration_all} plots the fraction of memory pages with no migration, exactly one migration, and more than one migration using Nimble's dynamic page migration policy for our evaluated workloads. 
\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/migration_summary.pdf}}
	\caption{Fraction of memory pages that suffer no migration, exactly one migration, and more than one migration using Nimble for our evaluated workloads.}
	\vspace{-10pt}
	\label{fig:migration_all}
\end{figure}
%\vspace{-6pt}

The number of migrations is counted considering the transitions of a memory page from cold-to-hot and vice-versa, resulting in re-allocation and de-allocation of the fast memory.  We observe a wide variation in behavior across these programs. For instance, over 93\% of memory pages in perlbench are migrated at most once, whereas 95\% of all pages in roms are migrated more than once. On average, 67\% of memory pages in these programs suffer more than one migration during their execution. These migrations lead to high energy and performance overhead.

Observation 2 leads to our \textbf{second key idea} that if a memory page is placed in a matching memory during its initially allocation, many of these migrations can be eliminated, leading to performance and energy improvement (Sec. \ref{sec:results}).

\noindent\textit{\underline{Observation 3}: There are typically only a few first-touch instructions in a program and only a small percentage of these instructions induce the most memory accesses.}

Figure \ref{fig:ftis} plots the FTIs and referenced pages per billion instructions of our evaluated workloads. We report total FTIs (outer first bar in each set) and the number of FTIs that touch pages which serve over 90\% of memory accesses (inner first bar). We also report the pages referenced per billion instructions (second bar). We observe that 1) there are very few FTIs per billion instructions of each workload, and 2) on average, only 17\% of FTIs in a program touch pages which serve over 90\% of memory accesses.

\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/ftis_summary.pdf}}
	\caption{First-touch instructions (FTIs) per billion instructions of our evaluated workloads.}
	\vspace{-10pt}
	\label{fig:ftis}
\end{figure}

%\vspace{-10pt}

Observation 3 leads to our \textbf{third key idea} of profiling FTIs based on number of accesses to memory pages they touch and using it to predict the access intensity of a new memory page.
%This idea together with our second idea (based on observation 2) places a new memory page in a matching memory node during its initial allocation, improving performance and energy. \textbf{Ideas 2 and 3 can be applied to both hybrid memory systems and mainstream DRAM-only systems.} In Section~\ref{sec:results}, we evaluate both these memory architectures and show improvements.
%Section~\ref{sec:mechanism} extends ideas 2 and 3 to incorporate idea 1 so that a newly referenced memory page can be allocated to a desired segment within a matching memory node.

% %\noindent\textit{Observation 3: At scaled technology nodes, a long bitline leads to non-uniform bias requirements of its non-volatile memory cells, causing cells that are closer to the current source having lower access latency but higher reliability degradation than those that are further away.}

% Our third observation and related idea is based on the internal architecture of a memory. In the following, we limit our discussions to NVMs, where each bit is represented by the resistance of a cell. 
% The resistance is read and programmed by driving current through the cell using a peripheral structure, which consists of the sense amplifier (to read) and the write driver (to write).
% A peripheral structure is several orders of magnitude larger than the size of a cell \cite{sandhu2018memory}. To amortize this large size, each peripheral structure in a bank is connected to many (typically 4096) NVM cells through a wire called a \textit{bitline}. 

% %\noindent\textit{Observation 3: The electrical load of a cell on a bitline is independent of the cell's distance from the peripheral circuit.}
% \noindent\textit{Observation 3: Long bitlines lead to low cost-per-bit in a NVM device, but introduce performance and reliability penalty.}

% %\noindent\textit{Observation 3: Long bitlines in a NVM device preset high electrical load to the peripheral circuit when reading and programming a bitline's NVM cells, increasing access latency.}

% %\noindent\textit{Observation 3: Long bitlines in a NVM device lead to non-uniform bias requirements of its cells, causing those that are closer to the current source having lower access latency but higher reliability degradation than ones that are further away.}






% Observation 3 leads to our \textbf{third key idea} of introducing isolation transistors on long bitlines in a NVM device to achieve low cost-per-bit, while allowing their lengths to appear shorter in order
% to achieve low latency and high reliability. 
% Figure \ref{fig:segments} show our proposed architecture (details in Section \ref{sec:architecture}), where each long bitline is split into two segments using isolation transistor: the the segment that is connected directly to the peripheral circuit is called the \textit{near segment}, whereas the other is called the \textit{far segment}. In this way, cells in the near segment can be accessed faster with lower bias voltage, i.e., with higher reliability. However, isolation transistors increase access latency of cells in the far segment, and impose additional bias requirement for the peripheral circuit, which lowers their reliability.

% This concept of tiering inside a memory device was first proposed for DRAM \cite{lee2013tiered}, where the authors show significant performance improvements. We extend the concept to NVM and address its performance and reliability tradeoffs.

% \begin{minipage}[h]{0.45\columnwidth}
% \centering
% 	%\vspace{-10pt}
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/segments.pdf}}
% 	%\vspace{-10pt}
% 	\captionof{figure}{Our proposal to segment long bitlines.}
% 	\label{fig:segments}
% \end{minipage}
% \begin{minipage}{0.48\columnwidth}
% \centering
% 	%\vspace{-10pt}
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/program_execution.pdf}}
% 	%\vspace{-10pt}
% 	\captionof{figure}{Program execution in our proposed architecture.}
% 	\label{fig:program_execution}
% \end{minipage}


%access latency and reliability characteristics

We introduce \textbf{\tech{}}\footnote{In Greek mythology, \tech{} is the muse of memory. \tech{} means persistent effect of memory of past events, which are the first-touch instructions in the context of this paper.}, 
a mechanism that
builds on the three ideas above to enable 
additional tiers in hybrid memories and exploit these tiers through OS-level page allocation policy.
\tech{} places a newly referenced memory page to the best tier during its initial allocation, minimizing channel and bank occupancy associated with migration of the page during execution. 
%This improves performance, reliability, and energy.
%and exploit inter- and intra-memory performance and reliability asymmetries in hybrid tiered-memories.
%an approach to allocate pages in a hybrid memory system, where each heterogeneous memory node has segmented bitlines, introducing latency and reliability asymmetries. 
Our \textbf{tiered-memory architecture} is shown in Figure~\ref{fig:tms}, where the tiers are arranged with increasing access latency from CPU.  Figure~\ref{fig:program_execution} shows a high-level overview of our page allocation policy to exploit this tiered architecture. A program is broken down into fixed intervals (called \emph{phases}). At each phase
we profile FTIs based on accesses to pages they touch.
% and use it to 
%  during each phase, we profile first-touch instructions of the program. 
This information is then used to decide the initial placement of all newly referenced memory pages of the subsequent phases.
%to the best memory tier, minimizing the migration of the page during execution.
% to a matching segment within a matching memory node

% \begin{figure}[t!]
% 	\centering
% 	%\vspace{-10pt}
% 	\centerline{\includegraphics[width=0.69\columnwidth]{images/program_execution.pdf}}
% 	\caption{Program execution in our proposed approach.}
% 	\vspace{-12pt}
% 	\label{fig:program_execution}
% \end{figure}

% This paper makes the following \textbf{contributions}.
% \begin{itemize}
%     \item We introduce a tiered-memory architecture with segmented bitlines within heterogeneous memories and analyze their performance and reliability trade-offs.
%     \item We propose an approach to predict access intensity of a new memory page using the page's first-touch instruction and 
%     %. We exploit the asymmetric latency and reliability characteristics to 
%     place it in the best memory tier, reducing its migration during program execution.
    
%     \item We develop our FTI-based page allocation for the entire program duration to adapt to and make correct allocation decisions for different phases of execution in a program with potentially distinct working sets.
%     %incorporate sudden changes in program execution phases.
    
%     \item We show how to reduce channel occupancy during page migration between tiers of the same memory, thereby improving performance.
    
%     \item We introduce efficient hardware implementation of \tech{} using Bloom filters.
    
%     \item We implement \tech{} for two different hybrid memory architectures and also for commodity DRAM-based mainstream architecture, and show significant performance and reliability improvement for both single-program and multi-programmed workloads.
% \end{itemize}

\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.69\columnwidth]{images/tms.pdf}}
	\caption{Proposed Hybrid Tiered-Memory Architecture.}
	\vspace{-10pt}
	\label{fig:tms}
\end{figure}

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.69\columnwidth]{images/program_execution.pdf}}
	\caption{Proposed program execution.}
	\vspace{-10pt}
	\label{fig:program_execution}
\end{figure}

%\vspace{5pt}
% \begin{minipage}[t]{0.5\columnwidth}
% \centering
% 	%\vspace{-10pt}
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/tms.pdf}}
% 	%\vspace{-10pt}
% 	\captionof{figure}{Proposed Hybrid Tiered-Memory Architecture}
% 	\label{fig:tms}
% \end{minipage}
% \begin{minipage}{0.5\columnwidth}
% \centering
% 	\vspace{-15pt}
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/program_execution.pdf}}
% 	%\vspace{-10pt}
% 	\captionof{figure}{Proposed program execution.}
% 	\label{fig:program_execution}
% \end{minipage}

%\vspace{5pt}

%We evaluate \tech{} using 

% \begin{figure}[h!]
% 	\centering
% 	%\vspace{-10pt}
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/program_execution.pdf}}
% 	\caption{Program execution in our proposed architecture.}
% 	%\vspace{-10pt}
% 	\label{fig:program_execution}
% \end{figure}

%an approach to predict the access intensity of memory pages and place them in matching memory nodes during their initial allocation, improving performance and 
